A Case for a Global Information Network

This paper argues for the adoption of a information centric system model instead of the current service-oriented one. We present an architecture for a global information storage and dissemination network which provides for efficient interaction and coordination among autonomous actors through a shared information space. We believe that the resulting, loosely coupled systems, while probabilistic in nature, will lead to robust outcomes at large scales.

==> discussion.tex <==
\section{Discussion}\label{discussion}

The GSG poses interesting research questions that provide an opportunity for further exploration into the GSG's core ideas and main concepts behind it.
\medskip\\
\textbf{Context - based pub/sub system.} The GSG provides context - based publish/subscribe service. The challenge is to provide this service in large - scale fully distributed environment.
\medskip\\
\textbf{Security.} Without a doubt security is a very crucial part of any system. In our research we are looking at a suitable security model for the GSG. Our preliminary discussion are around "Named Graphs" that perhaps can be used in GSG's context to describe security attributes of a subgraph. The main challenge is how to enforce it in a large scale distributed environment.  
\medskip\\
\textbf{Evaluation.} We envision GSG to operate on a scale of  trillions of tuples, with billions of concurrent
subscriptions/queries from millions of decoupled agents. Finding the right benchmark is tricky as GSG will serve multiple purposes, for example, some applications may treat it as a global storage, while others will take advantage of context-based pub/sub to facilitate more enhance services - what is the right metric? Perhaps there is not just one and each GSG - based service will require an evaluation benchmark.

